DeclareViT: Decoupling Early Classification from Feature Refinement with Exit Query for Efficient ViTs

Vision Transformers achieve remarkable recognition performance but incur substantial computational cost during inference, limiting their use in latency- and compute-constrained deployment scenarios. Early-exit inference offers a promising solution by allowing easy samples to terminate at intermediate layers. However, existing approaches typically couple early classification with the shared backbone, requiring intermediate representations to support both early classification and subsequent feature refinement. Under joint training, the corresponding optimization objectives jointly update shared backbone parameters, which can lead to conflicting gradient directions. Motivated by this observation, we introduce DeclareViT, a framework that decouples early classification from feature refinement. Each exit uses a dedicated query to read intermediate features through one-way cross-attention without modifying the backbone token stream. The query branches are optimized for early classification while the backbone and final classifier remain frozen. Across ViT, DeiT, and Swin on CIFAR-100, ImageNet-1K, and Food-101, DeclareViT consistently establishes a state-of-the-art accuracy-efficiency trade-off: It achieves 1.58 times to 2.57 times multiply-accumulate (MAC)-based speed-up with only a 0.39-1.91 percentage-point accuracy drop. Wall-clock measurements on CPU and GPU further demonstrate practical inference acceleration. Code is available at https://github.com/TUDa-HWAI/DeclareViT.

==> overview_layout.tex <==
% Load this file in the manuscript preamble.
\RequirePackage{graphicx}
\RequirePackage{tikz}
\providecommand{\AttentionAssetRoot}{artwork/attention}
\definecolor{AttentionHigh}{RGB}{253,231,36}

% Arguments: dataset folder, dataset display name, sample ID, class, attention limit, difference limit.
% The heatmaps are embedded unchanged; labels and colorbar ticks are native TeX.
\providecommand{\AttentionOverview}[6]{%
  \begingroup
  \resizebox{\linewidth}{!}{%
    \begin{tikzpicture}[x=1mm,y=1mm,
        every node/.style={inner sep=0,outer sep=0,
          font=\sffamily\fontsize{8}{9}\selectfont}]
      \path[use as bounding box] (0,0) rectangle (192,94);
      \node[anchor=south west] at (0,32)
        {\includegraphics[width=32mm]{\AttentionAssetRoot/#1/sample_#3/input.png}};
      \draw[black!70,line width=0.2pt] (0,32) rectangle (32,64);
      \node[anchor=south,align=center,text width=32mm] at (16,66)
        {\hyphenpenalty=10000 GT: #4\par};
      \foreach \column/\filedepth/\depth in {0/02/2,1/04/4,2/06/6,3/08/8,4/10/10}{%
        \pgfmathsetmacro{\panelx}{44+26*\column}
        \node at (\panelx+12,89) {@\depth};
        \foreach \kind/\panely in {cls/62,query/36,difference/10}{%
          \node[anchor=south west] at (\panelx,\panely)
            {\includegraphics[width=24mm]{\AttentionAssetRoot/#1/sample_#3/\kind_block\filedepth.png}};
          \draw[black!70,line width=0.2pt]
            (\panelx,\panely) rectangle (\panelx+24,\panely+24);
        }
      }
      \node[rotate=90] at (38,74) {Backbone CLS};
      \node[rotate=90] at (38,48) {Exit Query};
      \node[rotate=90] at (38,22) {Query $-$ CLS};

      % One probability scale for both attention rows, including upper clipping.
      \node[anchor=south west] at (175,36)
        {\includegraphics[width=2.5mm,height=50mm]{\AttentionAssetRoot/colorbars/viridis_strip.png}};
      \draw[line width=0.2pt] (175,36) rectangle (177.5,86);
      \filldraw[fill=AttentionHigh,line width=0.2pt]
        (175,86) -- (176.25,88) -- (177.5,86) -- cycle;
      \foreach \tickvalue in {0,0.02,0.04,0.06,0.08}{%
        \ifdim\tickvalue pt<#5pt\relax
          \pgfmathsetmacro{\ticky}{36+50*\tickvalue/(#5)}
          \draw[line width=0.2pt] (177.5,\ticky) -- (178.2,\ticky);
          \node[anchor=west,font=\sffamily\fontsize{7}{8}\selectfont] at (179,\ticky)
            {\pgfmathprintnumber[fixed,fixed zerofill,precision=2]{\tickvalue}};
        \fi
      }
      \node[anchor=west,font=\sffamily\fontsize{7}{8}\selectfont] at (179,86)
        {\pgfmathprintnumber[fixed,precision=3]{#5}};
      % \node[rotate=90,font=\sffamily\fontsize{7}{8}\selectfont] at (190,61)
      %   {Conditional patch attention};

      % Keep each sample's original symmetric difference limits.
      \node[anchor=south west] at (175,12)
        {\includegraphics[width=2.5mm,height=20mm]{\AttentionAssetRoot/colorbars/coolwarm_strip.png}};
      \draw[line width=0.2pt] (175,12) rectangle (177.5,32);
      \foreach \sign/\ticky in {-1/12,0/22,1/32}{%
        \pgfmathsetmacro{\value}{\sign*(#6)}
        \draw[line width=0.2pt] (177.5,\ticky) -- (178.2,\ticky);
        \node[anchor=west,font=\sffamily\fontsize{7}{8}\selectfont] at (179,\ticky)
          {\pgfmathprintnumber[fixed,fixed zerofill,precision=3]{\value}};
      }
      % \node[rotate=90,font=\sffamily\fontsize{7}{8}\selectfont] at (190,22)
      %   {Query $-$ CLS};
    \end{tikzpicture}%
  }%
  \endgroup
}

% Dataset plate: folder, display name, attention limit, sample count, sample inputs.
% Stack sample rows; each input carries its own ground-truth label.
\providecommand{\AttentionDatasetOverview}[5]{%
  \begingroup
  \def\AttentionPanelDataset{#1}%
  \def\AttentionPanelDatasetName{#2}%
  \def\AttentionPanelMaximum{#3}%
  \begin{minipage}{\linewidth}%
    \setlength{\parindent}{0pt}%
    \setlength{\parskip}{0pt}%
    \offinterlineskip
    #5%
  \end{minipage}%
  \endgroup
}

% Arguments: zero-based position, sample ID, class label, original difference limit.
\providecommand{\AttentionDatasetRow}[4]{%
  \ifnum#1>0\relax\vspace{3mm}\fi
  \noindent\AttentionOverview{\AttentionPanelDataset}{\AttentionPanelDatasetName}%
    {#2}{#3}{\AttentionPanelMaximum}{#4}\par
}

